Sensitivity of NEXT-100 to neutrinoless double beta decay

NEXT-100 is an electroluminescent high-pressure xenon gas time projection chamber that will search for the neutrinoless double beta ($\beta \beta 0 \nu$) decay of Xe-136. The detector possesses two features of great value for $\beta \beta 0 \nu$ searches: energy resolution better than 1\% FWHM at the $Q$ value of Xe-136 and track reconstruction for the discrimination of signal and background events. This combination results in excellent sensitivity, as discussed in this paper. Material-screening measurements and a detailed Monte Carlo detector simulation predict a background rate for NEXT-100 of at most $4\times10^{-4}$ counts keV$^{-1}$ kg$^{-1}$ yr$^{-1}$. Accordingly, the detector will reach a sensitivity to the \bbonu-decay half-life of $2.8\times10^{25}$ years (90\% CL) for an exposure of 100 $\mathrm{kg}\cdot\mathrm{year}$, or $6.0\times10^{25}$ years after a run of 3 effective years.

==> src/SensitivityNext100.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Sensitivity of NEXT-100}
%%%
The sensitivity of NEXT-100 to neutrinoless double beta decay --- calculated following the Feldman-Cousins prescription for the construction of confidence intervals \cite{Feldman:1997qc, GomezCadenas:2010gs} --- is shown in Figure~\ref{fig:SensitivityNEXT100}. In the top panel, the sensitivity (at 90\% CL) to the half-life (red, solid curve) and the corresponding sensitivity to \mbb\ (blue, dashed curves) for the largest and smallest NME calculations (see Table~\ref{tab:BBIsotopes}) are represented in terms of the exposure, assuming a signal detection efficiency of 28\% and a background rate of $6\times10^{-4}~\ckky$. The bottom panel shows, for an exposure of 100~kg$\cdot$year the variation of the sensitivity with respect to the background rate in the range between $10^{-5}$ and $10^{-4}$~\ckky.


%%%%%%%%%%
\begin{figure}
\centering
\includegraphics[width=0.75\textwidth]{img/Next100SensitivityVsExposure.pdf}
\includegraphics[width=0.75\textwidth]{img/Next100SensitivityVsBackground.pdf}
\caption{Sensitivity of NEXT-100 to neutrinoless double beta decay. Top: Sensitivity (at 90\% CL) to the \bbonu-decay half-life (red. solid curve) and the corresponding \mbb\ sensitivity (blue, dashed curves) for the largest and smallest NME calculations in terms of the exposure. Bottom: Sensitivity (at 90\% CL) in terms of the background rate.} \label{fig:SensitivityNEXT100}
\end{figure}
%%%%%%%%%%

